Benchmarking Learned Indexes

Recent advancements in learned index structures propose replacing existing index structures, like B-Trees, with approximate learned models. In this work, we present a unified benchmark that compares well-tuned implementations of three learned index structures against several state-of-the-art "traditional" baselines. Using four real-world datasets, we demonstrate that learned index structures can indeed outperform non-learned indexes in read-only in-memory workloads over a dense array. We also investigate the impact of caching, pipelining, dataset size, and key size. We study the performance profile of learned index structures, and build an explanation for why learned models achieve such good performance. Finally, we investigate other important properties of learned index structures, such as their performance in multi-threaded systems and their build times.

==> related.tex <==
\section{Related work}
\label{sec:rw}

Learned index structures were first introduced in~\cite{ml_index}, which included the RMI. Several works on learned index structures followed, including the RadixSpline index~\cite{radix-spline}, the PGM index~\cite{pgm-index}, FITing tree~\cite{fiting_tree}, and ALEX~\cite{alex}. This work evaluates RMIs, RadixSpline, and PGM, as public implementations of FITing tree and ALEX are not available. Flood~\cite{flood} extends learned index structures to multi-dimensional data, which is not considered in this work. In~\cite{lis_func_interp}, function interpolation is used to provide a light-weight, training-free approach to learned index structures.

It would be impossible to enumerate all prior works on index structures in general, so here we only highlight a few. ART~\cite{art}, HOT~\cite{hot}, and FST~\cite{surf} present optimized trie structures for indexing. FAST~\cite{fast} shows how architecture-specific optimizations, such as SIMD instructions, can be used to build optimized BTree-like structures. In~\cite{siptip}, the authors demonstrate that simple interpolation search techniques can often outperform binary search.  Several indexes have been explicitly designed for integration with LSM trees~\cite{lsm, lsm_survey}.
Besides ordered indexes, there are also many unordered or partially-ordered indexing approaches such as hash tables~\cite{hashing_eval,lsh1,lsh2,slimdb,faster,dash}. These techniques do not support lower bound lookups and thus cannot be applied to the problem studied in this work.

%\ak{Could drop related work section. It is not uncommon to not have related work in an E\&A paper. We are referencing most of these indexes throughout the paper anyways (especially in Section 5.1.1).}

% For the camera ready / arxiv:
%More broadly, work on learned indexes follows recent trends in integrating machine learning components into systems~\cite{pillars}, especially database systems. Machine learning techniques have also been applied to query optimization~\cite{neo, skinnerdb, qo_state_rep}, cardinality estimation~\cite{deep_card_est2, naru, plan_loss, deep_sketch, local_card_est}, cost modeling~\cite{learn_cost}, data integration~\cite{termite, deep_entity},tuning~\cite{ml_tuning}, security~\cite{sql_embed}, and workload management~\cite{wisedb-vldb, perfenforce}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

